Constraining the p{\Lambda} interaction from a combined analysis of scattering data and correlation functions

This work provides the first combined analysis of low-energy p$\Lambda$ scattering, considering both cross section and correlation data. The obtained results establish the most stringent constraints to date on the two-body p$\Lambda$ interaction, pointing to a weaker attraction than so far accepted. The best set of scattering lengths for the spin singlet and triplet are found to range from $f_0, f_1 = (2.1, 1.56)$ to $(3.34, 1.18)~$fm. With a chiral NY potential fine-tuned to those scattering parameters, the in-medium properties of the $\Lambda$ are explored and a potential depth of $U_\Lambda= -36.3\pm 1.3 \mathrm{(stat)}^{+2.5}_{-6.2}\mathrm{(syst)}$ MeV is found at nuclear matter saturation density.

==> Chapters/Summary.tex <==
\section{Summary and outlook}\label{sec:Summary}

We need to get there by December.\\
A realistic timeline:
\\~\\
\textbf{October:}\\
Johann evaluates several $U_\Lambda(\rho_0)$ values for the scattering parameters we circulated around. Goal: figure out what values we will roughly get, so that we know from the start our conclusions.\\
Dimitar finalizes the exclusion plot, I will run even more simulations if needed. Dimitar and Johann discuss if we need a "targeted" study of a specific f,d combinations, which should be easy to set up.\\
Valentina can start writing the introduction.
\\~\\
We should conclude the month by having cleared up all we want to write, in particular an estimate of our final results and conclusions.
\\~\\
\textbf{November:}\\
Dimitar and Johann do final iterations of whatever calculations are needed, in order to get the final results.\\
Johann starts writing chapter \ref{sec:pLambda}\\
Dimitar starts writing chapter \ref{sec:Analysis}\\
Valentina reviews the text to ensure consistency and starts preparing chapter \ref{sec:Summary}
\\~\\
\textbf{End-of-November and early December:}\\
We all write chapter \ref{sec:Results}, as it will be the most important one. We finalize \ref{sec:Summary}.\\
Finally, we all review the paper and aim to be on arxiv before mid-Dec

